Probabilistic Hyperproperties with Nondeterminism

We study the problem of formalizing and checking probabilistic hyperproperties for models that allow nondeterminism in actions. We extend the temporal logic \HyperPCTL, which has been previously introduced for discrete-time Markov chains, to enable the specification of hyperproperties also for Markov decision processes. We generalize HyperPCTL by allowing explicit and simultaneous quantification over schedulers and probabilistic computation trees and show that it can express important quantitative requirements in security and privacy. We show that HyperPCTL model checking over MDPs is in general undecidable for quantification over probabilistic schedulers with memory, but restricting the domain to memoryless non-probabilistic schedulers turns the model checking problem decidable. Subsequently, we propose an SMT-based encoding for model checking this language and evaluate its performance.

==> databaseprivacy.tex <==


{\em privacy in databases}~\cite{guarnieri2017} can be compromised indirectly  
indirectly when a user is able to infer confidential
data (for which he/she has not the right to access), by combining the query 
results with external information such as data dependencies 
or prior knowledge.

As example, let's consider the case of a database of a hospital or 
a medical center storing information about the smoking habits of 
patients and whether they have diagnosed with a lung cancer.  
The database contains four tables: \emph{patient} with all 
the names of the patients, \emph{smokes} containing all the 
names of the regular smokers, \emph{parent} indicating the 
name of each patient's parent that is also listed as patient
and the table \emph{cancer} with the names of the patient 
that have been diagnosed with the lung cancer. 
The last 


One table contains the name of all the patients, another 
all the names of the regular smokers. In addition we have other two 
tables: the first contains the names of all the  patients diagnosed 
with lung cancer and the second contains all the names of the 
parents of a specific patient. It is known 

[i Need to finish writing]

\todo{Ezio completes}



==> exists.tex <==
\section{Existential scheduler problems for MDPs and \PCTL}

Assume an MDP $\mdp$ having a label \emph{initial} to distinguish a unique 
initial state $\state\in \states$ with $\textit{initial}\in L(\state)$ and 
$\textit{initial}\notin L(\state')$ for all $\state'\in \states\setminus \{s\}$. 
According to the standard definition, the MDP in its initial state $s$  
satisfies a \PCTL property $\varphi$ iff for \emph{any} scheduler 
$\hscheduler_{\state}$ for $\mdp$, the DTMC $\mdp^{\hscheduler_{\state}}$ 
(induced by $\mdp$ and $\hscheduler_{\state}$) in state $s$ satisfies $\varphi$. 
This corresponds to the hyperproperty
\[
\forall \hstate. (\textit{initial}_{\hstate} \rightarrow 
(\forall\hscheduler_{\hstate}))
\]



==> figs/indpmc.tex <==
\begin{tikzpicture}
  \node[draw,circle] (s0) at (-2,1) {$s_0$};
  \node[node distance=5.2ex,left of = s0] {\footnotesize $\{h{>}0\}$};

  \node[draw,circle] (s1) at (2,1) {$s_1$};
  \node[node distance=5.2ex,right of = s1] {\footnotesize $\{h{\leq}0\}$};

  \node[draw,circle] (s2) at (-2,-1.5) {$s_2$};
  \node[node distance=5.2ex,left of = s2] {\footnotesize $\{l{=}1\}$};

  \node[draw,circle] (s3) at (2,-1.5) {$s_3$};
  \node[node distance=5.2ex,right of = s3] {\footnotesize $\{l{=}2\}$};

  %\node (n3) at (-2,-0.25) [circle,fill,inner sep=2pt]{};
  %\node (n4) at (-0.7,0.15) [circle,fill,inner sep=2pt]{};
  %\node (n1) at (0.7,0.15) [circle,fill,inner sep=2pt]{};
  %\node (n2) at (2,-0.25) [circle,fill,inner sep=2pt]{};

  \node (n5) at (2,-2.3) [circle,fill,inner sep=0.01pt]{};
  \node (n6) at (-2,-2.3) [circle,fill,inner sep=0.01pt]{};

\draw[-latex'] (s0)-- node[left,xshift=-2pt]{\footnotesize $\frac{2}{5} + \frac{7}{20} p_0$} (s2);

\draw[-latex'] (s0)-- node[right,pos=0,xshift=5pt,yshift=-1pt]{\footnotesize $\frac{3}{5} - \frac{7}{20} p_0$} (s3);
%\draw (s0)-- node[left]{\footnotesize $\alpha$} (n3);
%\draw[-latex'] (n3)-- node[left,pos=0.2,yshift=2pt]{\footnotesize $\frac{3}{4}$} (s2);
%\draw[-latex'] (n3)-- node[right,pos=0.05,yshift=4pt]{\footnotesize $\frac{1}{4}$} (s3);

%\draw (s0)-- node[right]{\footnotesize $\beta$} (n4);
%\draw[-latex'] (n4)-- node[left,pos=0.1,yshift=4pt]{\footnotesize $\frac{2}{5}$} (s2);
%\draw[-latex'] (n4)-- node[right,pos=0.05,yshift=4pt]{\footnotesize $\frac{3}{5}$} (s3);

\draw[-latex'] (s1)-- node[left,pos=0]{\footnotesize $\frac{1}{2} - \frac{1}{6} p_1$} (s2);
\draw[-latex'] (s1)-- node[right,xshift=2pt]{\footnotesize $\frac{1}{2} + \frac{1}{6} p_1$} (s3);

%\draw[-latex'] (n1)-- node[left,pos=0.05,yshift=4pt]{\footnotesize 
%$\frac{2}{3}$} (s2);
%\draw[-latex'] (n1)-- node[right,pos=0.1,yshift=4pt]{\footnotesize 
%$\frac{1}{3}$} (s3);

%\draw (s1)-- node[right]{\footnotesize $\beta$} (n2);
%\draw[-latex'] (n2)-- node[left,pos=0.05,yshift=4pt]{\footnotesize 
%$\frac{1}{2}$} (s2);
%\draw[-latex'] (n2)-- node[right,pos=0.2,yshift=2pt]{\footnotesize 
%$\frac{1}{2}$} (s3);
% \draw[-latex'] (s2)-- node[right,pos=0.2,yshift=-2pt]{\footnotesize 
% $\tau$} (n6);

% \draw[-latex', bend right] (s3)-- node[right,pos=0.2,yshift=-2pt]{\footnotesize 
% $\tau$} (n5);


\path (s3) edge[-, bend right] node[left,pos=0.2,yshift=-2pt] {\footnotesize 
} (n5);
\path (n5) edge[->, bend right] node[right,pos=0.2,yshift=3pt] {\footnotesize 
$1$} (s3);

\path (s2) edge[-, bend right] node[left,pos=0.2,yshift=-2pt] {\footnotesize 
} (n6);
\path (n6) edge[->, bend right] node[right,pos=0.2,yshift=3pt] {\footnotesize 
$1$} (s2);

% \path (s4) edge [loop below] node {\footnotesize $1$} (s4);

\end{tikzpicture}


==> logics.tex <==


\section{PCTL}

\begin{definition}[\PCTL syntax]
\emph{\PCTL state formulas} $\varphi$ and \emph{\PCTL path formulas}
$\psi$ over a countable set $\AP$ of atomic propositions are inductively defined by the following grammar:
\[
\begin{array}{lll}
\varphi & ::= & \tru \sep a \sep \varphi \wedge \varphi \sep \neg \varphi \sep \pr_{\sim c} (\psi) \\
\psi & ::= & \Next \varphi \sep  \varphi \, \U \, \varphi \sep  \varphi \, \U ^{[k_1,k_2]}\, \varphi  \\
\end{array}
\]
where $a \in \AP$,  $\sim \in \{<, \leq, \geq, >\}$, $c \in [0,1]\subseteq
\mathbb{Q}$  and $k_1,k_2\in\naturalszero$ with $k_1\leq k_2$. \emph{\PCTL
  formulas} are \PCTL state formulas.\hfill\qed
\end{definition}

\todo[inline]{Reminder: With the universal scheduler semantics, $\forall \scheduler.\pr_{= c} (\psi)$ and $\forall \scheduler.\pr_{\not= c} (\psi)$  can be expressed as below, thus we have all operators. The $4$ above are however needed: in order to express e.g. $\pr_{< c} (\varphi_1\U\varphi_2)$  using $\geq$, we need to express the probability of paths \emph{not} satisfying the until formula, which is the probability that $\varphi_2$ never gets true plus the probability that $\varphi_1$ is violated bevor $\varphi_2$ gets true. For a similar reason, $\varphi \, \U ^{[k_1,k_2]}\, \varphi$ can neither be expressed as syntactic sugar.}

\noindent 
We use parentheses as needed to denote the formula structure. We furthermore
introduce as syntactic sugar
\[
\begin{array}{l@{\quad}l@{\quad}l}
  \fals & \textit{for} & \neg \tru\\
  \varphi_1 \vee \varphi_2 & \textit{for} & \neg((\neg \varphi_1) \wedge (\neg\varphi_2))\\
  \varphi_1 \rightarrow \varphi_2 & \textit{for} & (\neg \varphi_1) \vee \varphi_2\\
  \varphi_1 \leftrightarrow \varphi_2 & \textit{for} & (\varphi_1 \rightarrow \varphi_2)\wedge(\varphi_2\rightarrow\varphi_1)\\
  \pr_{= c} (\psi) & \textit{for} & \pr_{\leq c} (\psi) \wedge \pr_{\geq c} (\psi)\\
  \pr_{\not= c} (\psi) & \textit{for} & \neg\pr_{=c} (\psi)\\
  \pr_{\sim c} (\varphi_1 \, \U^{\leq k} \,\varphi_2) & \textit{for} & \pr_{\sim c}(\varphi_1 \, \U^{[0,k]} \,\varphi_2)\\
  \pr_{\sim c}(\F \varphi) & \textit{for} & \pr_{\sim c}(\tru \, \U \, \varphi)\\
  \pr_{\sim c}(\F^{[k_1,k_2]} \varphi) & \textit{for} & \pr_{\sim c}(\tru \, \U^{[k_1,k_2]} \, \varphi)\\
  \pr_{\sim c}(\F^{\leq k} \varphi) & \textit{for} & \pr_{\sim c}(\tru \, \U^{\leq k} \, \varphi)\\
  \pr_{\sim c}(\G \varphi) & \textit{for} & \pr_{\overline{\sim} (1-c)}(\F\, (\neg \varphi))\\
  \pr_{\sim c}(\G^{[k_1,k_2]} \varphi) & \textit{for} & \pr_{\overline{\sim} (1-c)}(\F^{[k_1,k_2]}\, (\neg \varphi))\\
  \pr_{\sim c}(\G^{\leq k} \varphi) & \textit{for} & \pr_{\overline{\sim} (1-c)}(\F^{\leq k}\, (\neg \varphi))
\end{array}
\]
where $\varphi,\varphi_1,\varphi_2$ are PCTL state formulas, $\psi$ is a PCTL path formula, $k,k_1,k_2\in\naturalszero$ with $k_1\leq k_2$, and
$\overline{\sim}$ is $\geq, >, =, \not=, <, \leq$ for $\sim$ being
$\leq, <, =, \not=, >, \geq$, respectively. For Boolean operators we
assume the usual binding order
$\neg,\wedge,\vee,\rightarrow,\leftrightarrow$ from left to right.




The satisfaction of a \PCTL state (path) formula by a DTMC $\dtmc {=}
(\states, \P, \AP, L)$ is defined in the context of a
state (path) of $\dtmc$. In state formulas, the probability operator $\pr$ expresses that the probability of all paths
that start in the given state and fulfill a certain (path) property satisfies some bound. In path formulas, the next operator $\Next$ states that a property holds for the path when removing its first state. The until operator $\U$ states that the left operand holds until, after a finite number of steps, the right operand will be true.

\begin{definition}[\PCTL semantics for DTMCs]
For a DTMC $\dtmc {=} (\states, \P, \AP, L)$, the
satisfaction relation $\models$ defines the values of \PCTL
state and path formulas in the context of states $s\in \states$ respectively paths $\xpath\in\Paths{}{\dtmc}$  as follows:
\[
\begin{array}{lcl}
  \dtmc,\state \models \tru & \multicolumn{2}{l}{\textit{always}}\\
  \dtmc,\state \models a &
  \textit{iff} &
  a \in L(\state)\\
  \dtmc,\state  \models \varphi_1 \wedge \varphi_2 &
  \textit{iff} &
  \dtmc,\state \models \varphi_1 \textit{ and } \dtmc,\state  \models \varphi_2\\
  \dtmc,\state  \models \neg \varphi &
  \textit{iff} &
  \dtmc,\state \not \models \varphi\\
  \dtmc,\state\models \pr_{\sim c} \varphi & \textit{iff} & \Pr^{\dtmc}_{\state}(\{\xpath \in 
  \Paths{\state}{\dtmc} \mid \dtmc,\xpath \models \varphi\})\sim c\\
  \dtmc,\xpath \models \X \varphi &
  \textit{iff} &
  \dtmc,\xpath[1] \models \varphi\\
  \dtmc,\xpath \models \varphi_1 \U \varphi_2 &
  \textit{iff} &
  \exists j \geq 0. \Big(\dtmc,\xpath[j]\models\varphi_2 \wedge \forall i \in [0, j). \dtmc,\xpath[i] \models \varphi_1\Big)\\
  \dtmc,\xpath \models \varphi_1 \U^{[k_1,k_2]} \varphi_2 &
  \textit{iff} &
  \exists j \in [k_1,k_2]. \Big(\dtmc,\xpath[j]\models\varphi_2 \wedge \forall i \in [0, j). \dtmc,\xpath[i] \models \varphi_1\Big)
\end{array}
\]
\noindent for all $a \in \AP$, \PCTL state formulas $\varphi$,
$\varphi_1$, and $\varphi_2$,  $\sim \in \{<,
\leq, \geq, >\}$, $c \in \mathbb{Q}$ and $k_1,k_2\in\naturalszero$
with $k_1\leq k_2$.

\end{definition}

The \PCTL semantics for MDPs is similar but for the evaluation of
probability expressions we need to resolve non-determinism by a
scheduler. To evaluate a probability expression in a state $s$ of
$\mdp$ under a scheduler $\scheduler=(\modes, \act, \modef, \start)$,
we move to the DTMC induced by $\mdp$ and $\scheduler$ and consider
paths starting in the DTMC state
$\transup{\state,\scheduler}=(\state,\start(\state))$.  We will also use
$\transdown{\state',\mode'}= \state'$ to switch back from the context of
the induced DTMC to the context of the MDP.

\begin{definition}[\PCTL semantics for MDPs]
For an MDP $\mdp {=} (\states, \Act, \P, \AP, L)$, the
satisfaction relation $\models$ defines the values of \PCTL
state and path formulas in the context of states $s\in \states$ respectively paths $\xpath\in\Paths{}{\dtmc}$
by the following rules:
\[
\begin{array}{lcl}
  \mdp,\state \models \tru & \multicolumn{2}{l}{\textit{always}}\\
  \mdp,\state \models a &
  \textit{iff} &
  a \in L(\state)\\
  \mdp,\state  \models \varphi_1 \wedge \varphi_2 &
  \textit{iff} &
  \mdp,\state \models \varphi_1 \textit{ and } \mdp,\state  \models \varphi_2\\
  \mdp,\state  \models \neg \varphi &
  \textit{iff} &
  \mdp,\state \not \models \varphi\\
  %
  \mdp,\state\models \pr_{\sim c} \varphi & \textit{iff} & \forall \scheduler\in\schedulers{\mdp}.\Pr^{\mdp^{\scheduler}}_{\transup{\state,\scheduler}}(\{\xpath \in 
  \Paths{\transup{\state,\scheduler}}{\mdp^{\scheduler}} \mid \mdp,\xpath \models \varphi\})\sim c\\
  %
  \mdp,\xpath \models \X \varphi &
  \textit{iff} &
  \mdp,\transdown{\xpath[1]} \models \varphi\\
  %
  \mdp,\xpath \models \varphi_1 \U \varphi_2 &
  \textit{iff} &
  \exists j \geq 0. \Big(\mdp,\transdown{\xpath[j]}\models\varphi_2 \wedge \forall i \in [0, j). \mdp,\transdown{\xpath[i]} \models \varphi_1\Big)\\
    %
      \mdp,\xpath \models \varphi_1 \U^{[k_1,k_2]} \varphi_2 &
  \textit{iff} &
  \exists j \in [k_1,k_2]. \Big(\mdp,\transdown{\xpath[j]}\models\varphi_2 \wedge \forall i \in [0, j). \mdp,\transdown{\xpath[i]} \models \varphi_1\Big)\\
\end{array}
\]
\noindent for all $a \in \AP$, \PCTL state formulas $\varphi$,
$\varphi_1$, and $\varphi_2$, $\sim \in \{<, \leq, \geq, >\}$, $c
\in \mathbb{Q}$ and $k_1,k_2\in\naturalszero$ with $k_1\leq k_2$.

\end{definition}


\section{PCTL model checking for DTMCs}

The question whether a DTMC satisfies a PCTL property can be solved by
computing reachability probabilities. 
Assume a finite DTMC $\dtmc {=}
(\states, \P, \AP, L)$, a state $\state_0\in \states$ and a state set
$T\subseteq \states$.  We want to compute the probability
$\Pr^{\dtmc}_{\state_0}(\fPaths{\state_0,T}{\dtmc})$ to reach 
a state in $T$ when starting from $\state_0$ of $\dtmc$. 

%\ezio{Since we are considering DTMC, I think here it should be (by setting $\P(t,t)=1$ and $\P(t,\state)=0$, $\forall t\in T$ and $\state\in \states\setminus \{t\}$). Also why $\P(\state,\alpha,\state)=0$ ?}
First we make all states in $T$ absorbing (by setting
$\P(t,t)=1$ and $\P(t,\state)=\P(\state,t)=0$ for
all $t\in T$ and $\state\in \states\setminus
\{t\}$). 
%\ezio{I think $\states^- = \{ \state\in \states\suchthat\Pr^{\dtmc}_{\state}(\fPaths{\state,T}{\dtmc})=0\}$ }
Let $\states^- = \{ \state\in \states\suchthat
\Pr^{\dtmc}_{\state}(\fPaths{\state,T}{\dtmc})=0\}$ and $\states^+ = \{ \state\in \states\suchthat
\Pr^{\dtmc}_{\state}(\fPaths{\state,T}{\dtmc})=1\}$; note that these sets can be computed by
simple graph analysis. Assume $\state_0\notin \states^+\cup
\states^-$ (otherwise this probability is $1$ resp. $0$).


%\paragraph{State elimination}

%\begin{enumerate}

%\item \label{dtmc_selim:start} If $\states = \states^-\cup \states^+\cup\{\state_0\}$ then go to \ref{dtmc_selim:end}.

%\item Choose some $\state_2\in \states\setminus (\states^-\cup \states^+\cup\{\state_0\})$.

%\item If $\P(\state_2,\state_2)>0$ then for each $\state_3\in \states\setminus\{\state_2\}$ set $\P(\state_2,\state_3)$ to $\P(\state_2,\state_3)/\sum_{\state\in \states\setminus \{\state_2\}}\P(\state_2,\state)$, and set $\P(\state_2,\state_2)$ to $0$.

%\item For each $\state_1,\state_3\in \states\setminus\{\state_2\}$ increase $\P(\state_1,\state_3)$ by $\P(\state_1,\state_2)\cdot\P(\state_2,\state_3)$.

%\item For each $\state \in \states\setminus\{\state_2\}$ set $\P(\state,\state_2)$ and $\P(\state_2,\state)$ to $0$, set $\P(\state_2,\state_2)$ to $1$, add $\state_2$ to $\states^-$, and go to \ref{dtmc_selim:start}.

%\item \label{dtmc_selim:end} If $\P(\state_0,\state_0)>0$ then for each $\state\in \states\setminus\{\state_0\}$ set $\P(\state_0,\state)$ to $\P(\state_0,\state)/\sum_{\state'\in \states\setminus \{\state_0\}}\P(\state_0,\state')$, and set $\P(\state_0,\state_0)$ to $0$.

%\item The probability to reach $T$ from $\state_0$ is $\sum_{s\in \states^+}\P(\state_0,\state)/\sum_{s\in \states\setminus\{\state_0\}}\P(\state_0,\state)$.
  
%\end{enumerate}

\noindent\emph{Logical encoding}\quad Consider the linear equation system having a real-valued variable $p_{\state}$ 
for each $\state\in \states$ and consisting of (1) $p_{\state}=1$ for each $\state\in \states^+$; (2) $p_{\state}=0$ 
for each $\state\in \states^-$; (3) $p_{\state}=\sum_{\state'\in \states}\P(\state,\state')\cdot p_{\state'}$ for each 
$\state\in\states\setminus (\states^+\cup\states^-)$. This equation system has a unique solution, where the value 
of $p_{\state}$ equals $\Pr^{\dtmc}_{\state}(\fPaths{\state,T}{\dtmc})$ for each $\state\in\states$.

\noindent\emph{Value iteration}\quad We define $p_{\state}^{(0)}=1$ for each $\state\in\states^+$ and $p_{\state}^{(0)}=0$ for each $\state\in\states\setminus\states^+$, and let $p_{\state}^{(n+1)}=\sum_{\state'\in\states}\P(\state,\state')\cdot p_{\state'}^{(n)}$ for each $\state\in\states$ and $n\geq 0$. Then $\Pr^{\dtmc}_{\state}(\fPaths{\state,T}{\dtmc})=\lim_{n\rightarrow\infty} p_{\state}^{(n)}$ for each $\state\in \states$.

\section{PCTL model checking for MDPs}

Remember that an MDP satisfies a \PCTL property $\pr_{\sim c} (\psi)$ if for \emph{all}
schedulers their induced DTMCs satisfy the probability bound.  The question
whether an MDP satisfies a PCTL property can be solved by computing
minimal and maximal reachability probabilities. 
The following is a well-known result in the context of \PCTL 
model checking for MDPs.

\begin{lemma}[\cite{bk08-book}]
\label{lem:optial}
Let $\mdp= (\states, \Act, \P, \AP, L)$ be a finite MDP, $\state_0\in
\states$ and $T\subseteq\states$.  Then there exist memoryless deterministic
schedulers $\minscheduler,\maxscheduler\in\schedulers{\mdp}$ such that
$\Pr^{\mdp^{\minscheduler}}_{\state_0}(\fPaths{\state_0,T}{\mdp^{\sigma_*}})\leq
\Pr^{\mdp^{\scheduler}}_{\state_0}(\fPaths{\state_0,T}{\mdp^{\scheduler}})\leq
\Pr^{\mdp^{\maxscheduler}}_{\state_0}(\fPaths{\state_0,T}{\mdp^{\sigma^*}})$ for
all $\scheduler\in\schedulers{\mdp}$.  \hfill\qed
\end{lemma}


\noindent First we discuss how to determine \emph{minimal} reachability
probabilities.  Let $\mdp$, $\state_0$ and $T$ be as in the lemma
above.  Let $\states^- = \{ s\in \states\suchthat \exists
\scheduler\in\schedulers{\mdp}.\ \Pr^{\mdp^\scheduler}_{\state}(\fPaths{\state,T}{\mdp^{\scheduler}})=0\}$
and $\states^+ = \{ s\in \states\suchthat \forall
\scheduler\in\schedulers{\mdp}.\ \Pr^{\mdp^\scheduler}_{\state}(\fPaths{\state,T}{\mdp^{\scheduler}})=1\}$;
note that these sets can be computed by graph analysis.




We want to compute under all schedulers
$\scheduler\in\schedulers{\mdp}$ the minimal probability to reach a
state from $T$ in $\mdp^{\scheduler}$ when starting in $\state_0$ . Assume
$\state_0\notin \states^+\cup \states^-$ (otherwise this probability is $1$ resp. $0$).

\medskip

\noindent\emph{Logical encoding}\quad Consider the linear optimization problem to maximize $\sum_{\state\in\states}p_{\state}$ under the side conditions (1) $p_{\state}=1$ for each $\state\in \states^+$; (2) $p_{\state}=0$ for each $\state\in \states^-$; (3) $0\leq p_{\state}\leq 1$ and $p_{\state}\leq\sum_{\state'\in \states}\P(\state,\alpha,\state')\cdot p_{\state'}$ for each $\state\in\states\setminus(\states^+\cup\states^-)$ and $\alpha\in\Act(\state)$. For the unique optimum, the value of $p_{\state}$ for each $\state\in\states$ is the minimal probability (under all schedulers) to reach a state from $T$ when starting in state $\state$ of $\mdp$.

\medskip

\noindent\emph{Value iteration}\quad Let $p_{\state}^{(0)}=1$ for each $\state\in\states^+$, $p_{\state}^{(0)}=0$ for each $\state\in\states\setminus\states^+$, and $p_{\state}^{(n+1)}=\min_{\alpha\in\Act(\state)}\{\sum_{\state'\in\states}\P(\state,\alpha,\state')\cdot p_{\state'}^{(n)}\suchthat\alpha\in\Act(\state)\}$ for each $\state\in\states$ and $n\geq 0$. Then $\Pr^{\mdp^{\sigma_*}}(\fPaths{\state,T}{\mdp^{\sigma_*}}) = \lim_{n\rightarrow\infty} p_{\state}^{(n)}$ for each $\state\in \states$.

\medskip

\noindent To compute \emph{maximal} reachability probabilities, we modify the above descriptions setting Let $\states^- = \{ s\in \states\suchthat \forall
\scheduler\in\schedulers{\mdp}.\ \Pr^{\mdp^\scheduler}(\fPaths{\state,T}{\mdp^{\scheduler}})=0\}$
and $\states^+ = \{ s\in \states\suchthat \exists
\scheduler\in\schedulers{\mdp}.\ \Pr^{\mdp^\scheduler}(\fPaths{\state,T}{\mdp^{\scheduler}})=1\}$, and replacing maximum by minimum and vice versa at all places.

\section{The Temporal Logic \HyperPCTL for Probabilistic Hyperproperties of 
DTMCs~\cite{ab18}}
\label{subsec:hpctl}

\begin{definition}[\HyperPCTL syntax]
\emph{\HyperPCTL state formulas} $\varphi$ are inductively defined by the following 
grammar:
\[
\begin{array}{lll}
\varphi & ::= & \forall \hstate.\varphi \sep \exists 
\hstate.\varphi \sep \tru \sep a_{\hstate} \sep \varphi \wedge \varphi \sep \neg 
\varphi \sep p< p \\
\\
p & ::= & \pr(\psi) \sep c \sep p+p \sep  p-p 
\sep p\cdot p
\end{array}
\]
where $\hstate$ is a {\em state variable} from a countably 
infinite supply of variables $\hstates=\{\hstate_1,\hstate_2,\ldots\}$, $a \in \AP$ is an atomic proposition, $p$ is 
a \emph{probability expression}, $c \in \mathbb{Q}$,  and $\psi$ is a {\em \HyperPCTL path formula} defined by the grammar:
\[
\begin{array}{lll}
\psi & ::= & \Next \varphi \sep \varphi \, \U \, \varphi
\sep \varphi \, \U^{[k_1,k_2]} \,\varphi
\end{array}
\]
where $\varphi$ is a state formula  and $k_1, k_2 \in \naturalszero$ with $k_1\leq 
k_2$.

An occurrence of an indexed atomic proposition $a_{\hstate}$ in a \HyperPCTL 
state formula $\varphi$ is \emph{free} if it is not in the scope of a quantifier 
bounding $\hstate$ and otherwise \emph{bound}.
\HyperPCTL \emph{sentences} are \HyperPCTL state formulas
in which all occurrences of all indexed atomic propositions are bound.
\HyperPCTL (\emph{quantified}) \emph{formulas} are \HyperPCTL
sentences forming the set $\Phi$.

\end{definition}



\noindent 
We use parentheses as needed to denote the formula structure. We furthermore
introduce as syntactic sugar
\begin{center}
  \begin{tabular}{l@{\quad\quad}l}
    $
    \begin{array}{l@{\quad}l@{\quad}l}
      \fals & \textit{for} & \neg \tru\\
      \varphi_1 \vee \varphi_2 & \textit{for} & \neg((\neg \varphi_1) \wedge (\neg\varphi_2))\\
      \varphi_1 \rightarrow \varphi_2 & \textit{for} & (\neg \varphi_1) \vee \varphi_2\\
      \varphi_1 \leftrightarrow \varphi_2 & \textit{for} & (\varphi_1 \rightarrow \varphi_2)\wedge(\varphi_2\rightarrow\varphi_1)\\
%      p\in [l,u] & \textit{for} & l\leq p \wedge p \leq u\\
      p_1=p_2 & \textit{for} & \neg (p_1<p_2 \vee p_2<p_1)\\
      p_1\not= p_2 & \textit{for} & \neg(p_1=p_2)\\
      p_1\leq p_2 & \textit{for} & p_1<p_2 \vee p_1=p_2\\
      p_1\geq p_2 & \textit{for} & p_2\leq p_1\\
      p_1> p_2 & \textit{for} & p_2<p_1\\
    \end{array}
    $
&
    $
    \begin{array}{l@{\quad}l@{\quad}l}
      \pr(\varphi_1 \, \U^{\leq k} \,\varphi_2)\sim c & \textit{for} & \pr(\varphi_1 \, \U^{[0,k]} \,\varphi_2)\\
      \pr(\F \varphi) & \textit{for} & \pr(\tru \, \U \, \varphi)\\
      \pr(\F^{[k_1,k_2]} \varphi) & \textit{for} & \pr(\tru \, \U^{[k_1,k_2]} \, \varphi)\\
      \pr(\F^{\leq k} \varphi) & \textit{for} & \pr(\tru \, \U^{\leq k} \, \varphi)\\
      \pr(\G \varphi) & \textit{for} & 1-\pr(\F\, (\neg \varphi))\\
      \pr(\G^{[k_1,k_2]} \varphi) & \textit{for} & 1-\pr(\F^{[k_1,k_2]}\, (\neg \varphi))\\
      \pr(\G^{\leq k} \varphi) & \textit{for} & 1-\pr(\F^{\leq k}\, (\neg \varphi))\\\\
    \end{array}
    $
  \end{tabular}
\end{center}
where
%$l,u\in\mathbb{Q}$ are rational numbers,
$\varphi,\varphi_1,\varphi_2$ are \HyperPCTL state formulas, $p_1,p_2$ are probability expressions, and $k,k_1,k_2\in\naturalszero$ with $k_1\leq k_2$. For Boolean operators we
assume the usual binding order
$\neg,\wedge,\vee,\rightarrow,\leftrightarrow$ from left to right.


The probability operator $\pr$ is
similar to the one in \PCTL, but \PCTL
allows only the comparison of these probabilities to constant
thresholds, whereas \HyperPCTL allows the arbitrary usage of such
probabilities in arithmetic constraints. Another key difference
between \PCTL and \HyperPCTL is the quantification over (initial)
states to express probabilistic hyperproperties, i.e. to argue about
simultaneous executions in a Markov model.


The semantics of \HyperPCTL is based on $n$-ary {\em self-composition} 
of a DTMC.

\begin{definition}
The \emph{n-ary self-composition} of a DTMC $\dtmc = (\states, \P, \AP, L)$ is 
defined by the DTMC $\dtmc^n = (\states^n, \P^n, \AP^n, L^n)$, where

\begin{itemize}

\item $\states^n=\states\times\ldots\times \states$ is the $n$-ary Cartesian product of $\states$,

\item $\P^n\big(\state, \state')=\P(\state_1,\state_1'\big)\cdot\ldots\cdot \P(\state_n,\state_n')$ for 
all $\state=(\state_1,\ldots,\state_n)\in \states^n$ and $\state'=(\state_1',\ldots,\state_n')\in \states^n$,

\item $\AP^n=\cup_{i=1}^n\AP_i$ with $\AP_i=\{a_i\suchthat a\in\AP\}$ for $i 
\in [1, n]$, and

\item $L^n(\state) = \cup_{i=1}^n L_i(\state_i)$ for all $\state = (\state_1,\ldots,\state_n)\in \states^n$ 
with $L_i(\state_i) = \{a_i\suchthat a\in L(\state_i)\}$ for $i \in [1, n]$.\hfill\qed
\end{itemize}

\end{definition}

\noindent The satisfaction of a \HyperPCTL quantified formula by a DTMC $\dtmc 
{=} (\states, \P, \AP, L)$ is defined by:
\[
\dtmc \models \varphi \qquad 
\textit{iff} \qquad
\dtmc,()\models\varphi
\]
\noindent where $()$ is the empty sequence of states.  Thus, the meaning of a \HyperPCTL state
formula is defined in the context of a DTMC $\dtmc = (\states, \P, \AP, L)$ and a tuple 
$\state=(\state_1,\ldots,\state_n)\in \states^n$ of states (which is $()$ for $n=0$). Intuitively, 
the state sequence $\state$ stores instantiations for quantified state variables.  
The semantics evaluates \HyperPCTL formulas by structural recursion. 
Quantifiers are instantiated and the instantiated values for state variables 
are stored in the state sequence $\state$. To maintain the connection between a 
state in this sequence and the state variable which it instantiates, we 
introduce the auxiliary syntax $a_i$ with $a\in\AP$ and $i \in \naturals$, and 
if we instantiate $\hstate$ in
$\exists\hstate.\varphi$ or $\forall\hstate.\varphi$ by state $\state$, then we append $\state$ 
at the end of the state sequence and replace all $a_{\hstate}$ that is bound by 
the given quantifier by $a_i$ with $i$ being the index of $\state$ in the state 
sequence. The semantics judgment rules to evaluate formulas in the context of a 
DTMC $\dtmc = (\states, \P, \AP, L)$ and an $n$-tuple 
$\vstate=(\state_1,\ldots,\state_n)\in \states^n$ of states are the following:
\[
\begin{array}{l@{\quad}c@{\quad}l}
\dtmc,\vstate \models \forall \hstate.\varphi & 
\textit{iff} & 
\forall \state_{n+1} \in \states.\ \dtmc,(\state_1,\ldots,\state_n, \state_{n+1}) \models 
\varphi[\AP_{n+1}/\AP_{\hstate}]\\
\dtmc,\vstate \models \exists \hstate.\varphi & 
\textit{iff} & 
\exists \state_{n+1} \in \states.\ \dtmc,(\state_1,\ldots,\state_n, \state_{n+1}) \models 
\varphi[\AP_{n+1}/\AP_{\hstate}]\\
\dtmc,\vstate \models \texttt{true} &
 &
\\
\dtmc,\vstate \models a_i &
\textit{iff} &
a \in L(\state_i)\\
\dtmc,\vstate  \models \varphi_1 \wedge \varphi_2 &
\textit{iff} &
\dtmc,\vstate \models \varphi_1 \textit{ and } \dtmc,\vstate  \models \varphi_2\\
\dtmc,\vstate  \models \neg \varphi &
\textit{iff} &
\dtmc,\vstate \not \models \varphi\\
\dtmc,\vstate \models p_1 < p_2 &
\textit{iff} &
\llbracket p_1\rrbracket_{\dtmc,\vstate} < \llbracket p_2 \rrbracket_{\dtmc,\vstate}\\
\llbracket \pr(\psi)\rrbracket_{\dtmc,\vstate} & = & \Pr^{\dtmc^n}_{\vstate}(\{\xpath \in 
\Paths{\vstate}{\dtmc^n} \mid \dtmc,\xpath \models \psi\})\\
\llbracket c\rrbracket_{\dtmc,\vstate} & = & c\\
\llbracket p_1+p_2\rrbracket_{\dtmc,\vstate} & = & \llbracket p_1\rrbracket_{\dtmc,\vstate} 
+ \llbracket p_2\rrbracket_{\dtmc,\vstate}\\
\llbracket p_1-p_2\rrbracket_{\dtmc,\vstate} & = & \llbracket p_1\rrbracket_{\dtmc,\vstate} 
- \llbracket p_2\rrbracket_{\dtmc,\vstate}\\
\llbracket p_1\cdot p_2\rrbracket_{\dtmc,\vstate} & = & \llbracket 
p_1\rrbracket_{\dtmc,\vstate} \cdot \llbracket p_2\rrbracket_{\dtmc,\vstate}
\end{array}
\]
\noindent where $\varphi, \varphi_1,\varphi_2$ are \HyperPCTL state formulas, 
the substitution  $\varphi[\AP_{n+1}/\AP_{\hstate}]$ replaces for each 
atomic proposition $a\in\AP$ each free occurrence of $a_{\hstate}$ in $\varphi$ by
$a_{n+1}$, $a\in\AP$ is an atomic proposition, $i\in\{1,\ldots,n\}$, $p_1,p_2$ are probability expressions,
$\psi$ is a \HyperPCTL path formula, and $c$ is a rational constant.

The satisfaction relation for \HyperPCTL path formulas is defined as follows, 
where $\xpath$ is a path of $\dtmc^n$ for some $n\in\naturals$; $\varphi$, $\varphi_1$, 
and $\varphi_2$ are \HyperPCTL state formulas and $k_1,k_2\in\naturalszero$ with 
$k_1\leq k_2$:
\[
\begin{array}{l@{\quad}c@{\quad}l}
\dtmc,\xpath \models \X \varphi &
\textit{iff} &
\dtmc,\xpath[1] \models \varphi\\
\dtmc,\xpath \models \varphi_1 \U \varphi_2 &
\textit{iff} &
\exists j \geq 0. \Big(\dtmc,\xpath[j]\models\varphi_2 \wedge \forall i \in [0, j). 
\dtmc,\xpath[i] \models \varphi_1\Big)\\
\dtmc,\xpath \models \varphi_1 \U^{[k_1,k_2]} \, \varphi_2 &
\textit{iff} &
\exists j \in [k_1, k_2]. \Big(\dtmc,\xpath[j]\models\varphi_2 \; \wedge\; \forall i 
\in [0, j). \dtmc,\xpath[i] \models \varphi_1\Big)
\end{array}
\]

In~\cite{ab18}, we introduced an explicit-state model checking algorithm 
for verifying a DTMC $\dtmc$ against a \HyperCTL formula $\varphi$. The 
algorithm first constructs an $n$-ary self-composition of $\dtmc$, where 
$n$ is the number of quantifiers in $\varphi$ and the reduces the verification 
problem to \PCTL model checking. The complexity of the algorithm is 
polynomial-time in the size of $\dtmc$ and PSPACE-hard in the size of 
$\varphi$.



==> selfcomp.tex <==
    \begin{tikzpicture}

      \begin{scope}[xshift=-0.6cm,yshift=0cm]
        \node[anchor=east] (m) at (-0.25,0) {(a)\ $\mdp{:}$};
        
        \node[rectangle,inner sep = 1pt,draw] (s0) at (0,0) {$\state_0$};
        \node[rectangle,inner sep = 1pt,draw] (s1) at (-0.75,-1) {$\state_1$};
        \node[rectangle,inner sep = 1pt,draw] (s2) at (0.75,-1) {$\state_2$};

        \node[right of=s0,node distance=0.75cm] {\small $\{\textit{at0}\}$};
        \node[below of=s1,node distance=0.85cm] {\small $\{\textit{at1}\}$};
        \node[below of=s2,node distance=0.85cm] {\small $\{\textit{at2}\}$};
        
        \path[draw,-latex'] (s0) -- node[left,xshift=2pt]{$a$} node[right,xshift=-2pt]{$1$} (s1);
        \path[draw,-latex'] (s0) -- node[left,xshift=2pt]{$b$} node[right,xshift=-2pt]{$1$} (s2);
        \path[draw,-latex'] (s1) edge [loop below] node[left,xshift=0pt]{$c$} node[right,xshift=0pt]{$1$} (s1);
        \path[draw,-latex'] (s2) edge [loop below] node[left,xshift=0pt]{$c$} node[right,xshift=0pt]{$1$} (s2);
      \end{scope}
      
      \begin{scope}[xshift=3cm,yshift=0cm]
        \node[anchor=east] (m) at (-0.5,0) {(b)\ $\mdp^{\scheduler}_1{:}$};
        
        \node[rectangle,inner sep = 1pt,draw] (s0) at (0,0) {$(\mode,\state_0)$};
        \node[rectangle,inner sep = 1pt,draw] (s1) at (-0.75,-1) {$(\mode,\state_1)$};
        \node[rectangle,inner sep = 1pt,draw] (s2) at (0.75,-1) {$(\mode,\state_2)$};

        \node[right of=s0,node distance=1cm] {\small $\{\textit{at0}_1\}$};
        \node[below of=s1,node distance=0.85cm] {\small $\{\textit{at1}_1\}$};
        \node[below of=s2,node distance=0.85cm] {\small $\{\textit{at2}_1\}$};

        \path[draw,-latex'] (s0) -- node[right,xshift=-2pt]{$1$} (s1);
        \path[draw,-latex'] (s1) edge [loop below] node[right,xshift=0pt]{$1$} (s1);
        \path[draw,-latex'] (s2) edge [loop below] node[right,xshift=0pt]{$1$} (s2);
      \end{scope}
      
      \begin{scope}[xshift=3cm,yshift=-2.5cm]
        \node[anchor=east] (m) at (-0.5,0) {(c)\ $\mdp^{\scheduler'}_2{:}$};
        
        \node[rectangle,inner sep = 1pt,draw] (s0) at (0,0) {$(\mode',\state_0)$};
        \node[rectangle,inner sep = 1pt,draw] (s1) at (-0.75,-1) {$(\mode',\state_1)$};
        \node[rectangle,inner sep = 1pt,draw] (s2) at (0.75,-1) {$(\mode',\state_2)$};

        \node[right of=s0,node distance=1cm] {\small $\{\textit{at0}_2\}$};
        \node[below of=s1,node distance=0.85cm] {\small $\{\textit{at1}_2\}$};
        \node[below of=s2,node distance=0.85cm] {\small $\{\textit{at2}_2\}$};

        \path[draw,-latex'] (s0) -- node[right,xshift=-2pt]{$1$} (s2);
        \path[draw,-latex'] (s1) edge [loop below] node[right,xshift=0pt]{$1$} (s1);
        \path[draw,-latex'] (s2) edge [loop below] node[right,xshift=0pt]{$1$} (s2);
      \end{scope}

      \begin{scope}[xshift=7.7cm,yshift=-0.5cm]
        \node[anchor=east] (m) at (-1.2,0) {(d)\ 
$\mdp^{(\scheduler,\scheduler')}{:}$};
        
        \node[rectangle,inner sep = 1pt,draw] (s00) at (0,0) {$((\mode,\state_0),(\mode',\state_0))$};
        \node[rectangle,inner sep = 1pt,draw] (s12) at (0,-1.2) {$((\mode,\state_1),(\mode',\state_2))$};

        \node[rectangle,inner sep = 1pt,draw] (s01) at (3,0) {$((\mode,\state_0),(\mode',\state_1))$};
        \node[rectangle,inner sep = 1pt,draw] (s02) at (3,-1.2) {$((\mode,\state_0),(\mode',\state_2))$};
        \node[rectangle,inner sep = 1pt,draw] (s10) at (3,-2.4) {$((\mode,\state_1),(\mode',\state_0))$};
        \node[rectangle,inner sep = 1pt,draw] (s20) at (3,-3.6) {$((\mode,\state_2),(\mode',\state_0))$};

        \node[rectangle,inner sep = 1pt,draw] (s11) at (6,0) {$((\mode,\state_1),(\mode',\state_1))$};
        \node[rectangle,inner sep = 1pt,draw] (s21) at (6,-1.5) {$((\mode,\state_2),(\mode',\state_1))$};
        \node[rectangle,inner sep = 1pt,draw] (s22) at (6,-3) {$((\mode,\state_2),(\mode',\state_2))$};
        
        \node[above of=s00,node distance=0.4cm] {\small $\{\propof{\textit{at0}}{1},\propof{\textit{at0}}{2}\}$};
        \node[above of=s01,node distance=0.4cm] {\small $\{\propof{\textit{at0}}{1},\propof{\textit{at0}}{2}\}$};
        \node[above of=s02,node distance=0.4cm] {\small $\{\propof{\textit{at0}}{1},\propof{\textit{at0}}{2}\}$};
        \node[above of=s10,node distance=0.4cm] {\small $\{\propof{\textit{at1}}{1},\propof{\textit{at0}}{2}\}$};
        \node[above of=s11,node distance=0.4cm] {\small $\{\propof{\textit{at1}}{1},\propof{\textit{at1}}{2}\}$};
        \node[below of=s12,node distance=0.9cm] {\small $\{\propof{\textit{at1}}{1},\propof{\textit{at2}}{2}\}$};
        \node[above of=s20,node distance=0.4cm] {\small $\{\propof{\textit{at2}}{1},\propof{\textit{at0}}{2}\}$};
        \node[above of=s21,node distance=0.4cm] {\small $\{\propof{\textit{at2}}{1},\propof{\textit{at1}}{2}\}$};
        \node[above of=s22,node distance=0.4cm] {\small $\{\propof{\textit{at2}}{1},\propof{\textit{at2}}{2}\}$};

        \path[draw,-latex'] (s00) -- node[right,xshift=-2pt]{$1$} (s12);
        \path[draw,-latex'] (s01) -- node[above,xshift=-2pt]{$1$} (s11);
        \path[draw,-latex'] (s02) -- node[above,xshift=-2pt]{$1$} (s12);
        \path[draw,-latex'] (s10) -- node[below,xshift=-2pt]{$1$} (s12);
        \path[draw,-latex'] (s20) -- node[below,xshift=-2pt]{$1$} (s22);

        \path[draw,-latex'] (s11) edge [loop below] node[right,xshift=0pt]{$1$} (s11);
        
        \path[draw,-latex'] (s22) edge [loop below] node[right,xshift=0pt]{$1$} (s22);
        \path[draw,-latex'] (s12) edge [loop below] node[right,xshift=0pt]{$1$} (s12);
        \path[draw,-latex'] (s21) edge [loop below] node[right,xshift=0pt]{$1$} (s21);

      \end{scope}

    \end{tikzpicture}

